On margin-based generalization prediction in deep neural networks

Understanding generalization in deep neural networks is an active area of research. A promising avenue of exploration has been that of margin measurements: the shortest distance to the decision boundary for a given sample or that sample's representation internal to the network. Margin-based complexity measures have been shown to be correlated with the generalization ability of deep neural networks in some circumstances but not others. The reasons behind the success or failure of these metrics are currently unclear. In this study, we examine margin-based generalization prediction methods in different settings. We motivate why these metrics sometimes fail to accurately predict generalization and how they can be improved. First, we analyze the relationship between margins measured in the input space and sample noise. We find that different types of sample noise can have a very different effect on the overall margin of a network that has modeled noisy data. Following this, we empirically evaluate how robust margins measured at different representational spaces are at predicting generalization. We find that these metrics have several limitations and that a large margin does not exhibit a strong correlation with empirical risk in many cases. Finally, we introduce a new margin-based measure that incorporates an approximation of the underlying data manifold. It is empirically demonstrated that this measure is generally more predictive of generalization than all other margin-based measures. Furthermore, we find that this measurement also outperforms other contemporary complexity measures on a well-known generalization prediction benchmark. In addition, we analyze the utility and limitations of this approach and find that this metric is well aligned with intuitions expressed in prior work.

==> lists/acronymlist.tex <==
% This file contains all the acronyms used in the thesis and generates the list of acronyms.
% Clear the acronym memory...
\acresetall
\addcontentsline{toc}{chapter}{List of Abbreviations}
\chapter*{List of Abbreviations}
\begin{flushleft}

% Either all capitals matching abbreviation or all small except names
\begin{acronym}
\acro{DNN}{deep neural network}
% \acro{ReLU}{rectified linear unit}
% \acro{SGD}{stochastic gradient descent}
% \acro{KDE}{kernal density estimator}
% \acro{MSE}{mean squared error}
\acro{MLP}{multilayer perceptron}
% \acro{CLT}{computational learning theory}
\acro{GAN}{generative adversarial network}
\acro{CNN}{convolutional neural network}
\acro{PCA}{principal component analysis}
\acro{TV}{total variance}

\end{acronym}
\end{flushleft}

==> throwaway/ch6_CONCLUSION_OLD.tex <==

%\addbibresource{ref.bib}
\let\cite\parencite

% Headers & footers
\lhead{}
\rhead{}
\chapter{Conclusion}
\label{chap:conclusion}
% After chapter page reinstate default Headers & footers
\afterpage{\lhead{\ifthenelse{\thepage>0}
       {\it Chapter \thechapter }
      }
\rhead{\ifthenelse{\thepage>0}
       {\it \let\uppercase\relax\leftmark}
      }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\underline{ \hspace{\textwidth} } 
\textit{''It was over in a moment and the folks had gathered round \\
There before them lay the body of the outlaw on the ground \\
Oh, he might have went on living but he made one fatal slip \\
When he tried to match the ranger with the big iron on his hip''} \\ - Marty Robbins, \textit{Big Iron}, Verse 8\\
\underline{ \hspace{\textwidth} }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Overview}

Throughout this study, we have made many observations. In this chapter, we consolidate these findings, discuss these results, and also speculate on the remaining questions. 

The layout is as follows. We first list our key findings from each chapter in Section~\ref{sec:conclusion_key_findings}. We then move on to a discussion of these findings and also identify key questions for future work in Section~\ref{sec:conclusion_dicussion}. Our closing remarks are then contained in Section~\ref{sec:conclusion_in_closing}.

\section{Key findings and discussion}
\label{sec:conclusion_key_findings}

In this section, we very briefly summarize the idea of each experimental chapter. Following this, we list only the core findings. We then summarize the primary implications of these findings.

\textbf{Chapter 3: Margins and sample noise}

We investigate how margin measurements relate to different types of noisy samples. Specifically, we contrast the margins of clean, Gaussian-input-corrupted, and label-corrupted samples for a set of MLP and CNN models. Our core findings are as follows:

\begin{itemize}
    \item Standard input margins increase in size as model capacity increases. This is true for all of the different sample types.
    \item Label-corrupted samples have consistently smaller margins than clean samples. The presence of these samples also reduces the size of the margins of clean samples in the same model. 
    \item The proximity of a sample to the nearest sample of a different class (maximum margin) has some effect on the sample's margin.
\end{itemize}

The main implication of this is that mislabeled samples can drastically reduce the adversarial robustness of DNN models. Furthermore, we show that in this setting models of larger capacities have larger margins and are therefore more robust. Finally, the last finding provides some evidence for why some samples have larger margins than others. This is an important consideration for understanding how DNNs models noisy samples. 

\textbf{Chapter 4: Evaluating input and hidden margins
on PGDL}

In this chapter, we perform a large-scale evaluation of input and hidden margins on the PGDL dataset for the purpose of generalization prediction. We analyze margins in the context of numerical prediction and ranking of generalization. Furthermore, we perform ablation analysis on key design choices of these measurements. The core findings are as follows:

\begin{itemize}
    \item Standard input margins are not predictive of generalization, in general. This is true for both the numerical prediction and the ranking generalization settings.
    \item Hidden margins are more predictive of generalization than standard input margins. However, it is difficult to normalize hidden margins to be comparable between models with different architectural setups. The choice of hidden layer can have a very large effect on the performance.
    \item Combining DeepFool with a small learning rate enables it to find perturbations that are smaller than those of a constrained optimization formulation.
    \item Measuring standard input or hidden margins more accurately does not improve their performance.
\end{itemize}

The main implication of this chapter is that current margin-based complexity measures are brittle and that this is not due to poor approximation methods. Standard input margins tend not to be predictive at all, whereas hidden margins are subject to an essentially arbitrary hidden layer selection. 

\textbf{Chapter 5: Input margins can predict generalization too}

Lastly, in this chapter, we bridge the gap between input and hidden margins. We design a new complexity measure: constrained margins. This complexity measure incorporates standard input margins with the principal components of the dataset. This measurement is compared to other margin-based measures and complexity measures. Finally, we use this formulation to investigate adversarial examples. 

\begin{itemize}
    \item Constrained margins outperform standard input and hidden margins on the PGDL dataset.
    \item Constrained margins achieve the highest average performance on the PGDL test set compared to other complexity measures. 
    \item Constrained margins are still subject to certain limitations and have poorer performance on certain tasks compared to other complexity measures.
    \item Adversarial examples are found in the directions of the mid-tier principal components.
\end{itemize}

We have provided an intuitive reason why standard input margins do not accurately predict generalization. This argument is supported by strong empirical evidence. The implications of this are numerous. First, we show that the data manifold needs to be taken into account for future investigations between margins and generalization. Second, this opens up avenues of exploration for using constrained margins as a regularizer to improve the performance of DNNs. Finally, we have improved upon the current state-of-the-art (w.r.t. the PGDL challenge) for generalization prediction, with all of the benefits that entail. Recall our list of the many uses of complexity measures in Section~\ref{sec:intro_generalization}.  


\section{Discussion, speculation, and future work}
\label{sec:conclusion_dicussion}

We shall now discuss in more detail the findings and implications listed in the previous section. In addition, let us speculate a bit on that which we have not answered and identify avenues for future work.

\subsection{Core thesis}

First, let us consider our findings as a whole. The observations we have made throughout this study boil down to the following thesis: \textit{Margin measurements require an appropriate distance metric to be predictive of generalization in DNNs.} Let us explain the reasoning behind this. We have observed that margins measured in the input space using euclidean distance are not predictive of generalization. However, after a single non-linear transformation, these same measurements at the first hidden layer are much more correlated with generalization. Similarly, measuring the input space margin in a principal component subspace is also much more predictive of generalization. 

We know that constraining the search to a warped subspace and using Euclidean distance to measure closeness is equivalent to defining a new distance metric on the original space. This implies that, ultimately, we are seeking a relevant distance metric to measure the closeness of the decision boundary. Understanding the requirements for such a metric remains an open question. The positive results achieved with the current PCA-and-Euclidean-based approach of constrained margin provide strong motivation that this is a useful avenue to pursue.% Unfortunately, this is made difficult as current approximations and methods for finding points on the decision boundary are largely confined to $L_p$ metrics. 

We shall now consider some remaining questions and points of discussion from this distance metric perspective. We do not limit our focus here to only generalization prediction, but also to how the choice of distance metric relates to some of the other key observations.

\subsubsection{Why are hidden margins predictive of generalization?}

We have provided a strong argument and evidence for the question, `why are standard input margins not predictive of generalization?' However, we have not answered `why are hidden margins more predictive?'  We suspect that a plausible reason for this is that the non-linear transformations of the hidden layers act as a `feature selector'. These transformations are done in such a way that Euclidean measurements in this space are more aligned with the underlying data manifold of the input space. 

To investigate the correspondence between the hidden and input space, one could simply map points found on the decision boundary in the hidden space back to the input space. These points can then be visually inspected to determine whether there is truth to this hypothesis. Very recent work by Youzefsadeh~\cite{yousef_paths} shows that in the case of MLPs, it is possible to map points in the hidden space back to points in the input space. However, we have thus far been unable to reproduce this~\footnote{This is ongoing work and not shown in this study.} for the CNNs that we investigated throughout this study. This requires further study.

% Similar to the question posed above, we have also not answered `why are standard input margins predictive of generalization in some cases?' Recall that

\subsubsection{Sample specific margin behavior}

This lens of appropriate distance metric also allows us to discuss sample specific margin behavior.  Recall that in Chapter $3$ (specifically, Section~\ref{sec:noise_analysis}) we find a weak relationship between the margin of each sample and its Euclidean distance to the nearest sample of a different class (i.e. its maximum margin). However, we do not satisfactorily answer why some samples have smaller margins than others. On the other hand, at the end of Chapter $5$ (Section~\ref{sec:constrained_adv_dirs_results}) we find that standard input margins (i.e. adversarial examples) are mostly measured in the directions of the mid-tier principal components. It is thus possible that the proximity of the samples to each other in these directions has a greater effect on their respective margins than Euclidean distance over the entire space. This is an important consideration for gaining a better understanding of how noisy samples influence the margin, and thus generalization and robustness behavior, of DNNs. We are eager to investigate this hypothesis.

\subsubsection{Margin maximization}
 
 Let us consider how these findings relate to margin maximization methods. Several authors have developed techniques to maximize standard input~\cite{xu2023exploring} and hidden~\cite{large_margin_dnns} margins during training; however, these have not resulted in improved generalization. This raises the question of whether maximizing constrained margins would produce a different effect. We believe that constrained margin has the potential of being a powerful regularizer, in line with how other complexity measures have been used in the past. Furthermore, one could also consider adversarial retraining as a margin maximization method. Given that adversarial retraining generally results in reduced generalization, does that imply that adversarial retraining increases the standard input margin but reduces the constrained margin? It is possible that an increase in margin in one direction of the input space results in a decrease in margin in another direction. This is a promising direction for future investigations. 

\subsubsection{Improving constrained margin}

We must not forget that the constrained margin complexity measure we have presented is not without limitations.  In Section~\ref{sec:constrained_limitations} we discuss these in detail. Of great interest are certain PGDL tasks for which the metric performs worse than other complexity measures. We speculate that for these tasks the principal components are not a good approximation of the underlying data manifold. This implies that constrained margins are not an optimal distance metric for these tasks.

A natural next step is to establish whether the predictive performance of constrained margins can be improved if a more advanced manifold approximation measure is used. This is unfortunately difficult as it is infeasible to combine our approximation methods (the first-order Taylor approximation or DeepFool) with non-linear dimensionality reduction techniques. Furthermore, we have not established why networks with different depths appear to have different constrained margin behaviors. It is thus necessary to establish what effect certain architectural choices have on the model's margins.

\subsection{Other observations}

In addition to our core arguments, there are two other interesting observations that merit discussion. 

First, we have noticed that the accuracy of a margin-approximation method does not seem to be very important for the purpose of comparing summary statistics. Recall that at the end of Chapter $3$ (Section~\ref{sec:noise_hidden_margins}) we observed that the mean first-order Taylor approximated margins gave very similar results to the mean constrained optimization margins. Furthermore, we show in Chapter $4$ (Section~\ref{sec:hidden_df_pgdl_results}) that the predictive performance of standard input and hidden margins is not improved when using a more accurate method. This implies that, at least for some use cases, one need not be too concerned about the accuracy of the estimation method. This is interesting, as much of the literature surrounding classification margins is primarily concerned with the arms race of developing better margin finding methods.

Second, in a contradictory fashion to that stated above, we do find it very interesting that combining DeepFool with a small learning rate leads to finding a measurably smaller margin. This is an important consideration for the future design of white-box adversarial attacks. We have not compared this to other techniques such as the Fast Adaptive Boundary (FAB) attack, but perhaps this finding can lead to the design of improved approximation methods.

% Finally, we have also observed that in some cases, standard input margins are somewhat predictive of generalization.  

\section{In closing}
\label{sec:conclusion_in_closing}

In conclusion, we are searching for an appropriate distance metric to relate margin measurements to the generalization of deep neural networks. In this study, we have gained a better understanding of the requirements for such a metric. However, there is still much unanswered.

And now, dear reader, our time together comes to an end. It is our hope that you have enjoyed margins as much as we have.

==> throwaway/scratchpad.tex <==
Youzefsadeh and O'Leary~\cite{constrained_optim_investigating} introduce 'flip points', the point at which the classification of a sample flips from one class to another, i.e. a point on the decision boundary. Instead of relying on approximate methods, they formulate finding such a point as a constrained optimization problem, and then solve it using an off-the-shelf-optimizer. For example, the class of optimization methods found in the NLOpt software package. While this method is more precise, it comes at a great computational cost for high-dimensional input data (such as natural images), to alleviate this, dimensionality reduction methods are used prior to model training~\cite{constrained_optim_investigating}. They further show that the decision boundaries of a trained DNN have high curvature. In addition, they find that there exists a connected same-class-classification-region between samples of the same class. These two conclusions were also reached earlier by Fawzi et al.~\cite{fawzi_curvature} (albeit using different methods), who additionally find that networks are most vulnerable to adversarial perturbations in directions of high curvature. Follow up work by Youzefsadeh and O'Leary relates flip points to network interpretability~\cite{constrained_optim}.

Somepalli et al.~\cite{twice_dd_real_ver} visualize the classification regions within a plane spanned by three training examples in order to study the decision boundary characteristics of different models. They find that models within the same architecture group have visually similar classification regions, while there are greater dissimilarities between architectures with different forms of inductive bias (e.g. CNNs compared to vision transformers).  Furthermore, in order to study the double descent phenomenon~\cite{nakkiran_dd}, the margins of normal and label-corrupted training examples are measured by using a simple bisection search in ten random directions from each training sample. %Maybe something here about the fragmentation they observed, although it's not really relevant to anything in this study.  

Several authors have measured decision boundary characteristics by simply linearly interpolating between samples. Guan and Loew~\cite{guan_linear_interpol} utilize this method to define a measure of decision boundary complexity, and argue that a simpler decision boundary indicates greater generalization.  Although, the empirical evidence is limited to using two simple datasets, and only comparing two models per dataset. Karimi et al.~\cite{deep_dig} introduce \textbf{Deep} \textbf{D}ecision boundary \textbf{I}nstance \textbf{G}eneration (DeepDIG), an autoencoder based method to generate samples on or near the decision boundary. Using this method, the decision boundary complexity is described by generating two decision boundary samples and linearly interpolating between them. The complexity is then given by the rate of classification-oscillation along this path, meaning how many times the model classification changes. However, no clear relationship is demonstrated between this complexity and generalization.

%@inproceedings{missing_margin,
  %title={{The Missing Margin: How Sample Corruption Affects Distance to the Boundary in %ANNs}},
%  author={Theunissen, Marthinus Wilhelmus and Mouton, Coenraad and Davel, Marelie H},
%  booktitle={Southern African Conference for Artificial Intelligence Research},
%  pages={78--92},
%  year={2022},
%  organization={Springer}
%}

